The Effect of Flagella Stiffness on the Locomotion of a Multi-Flagellated Robot at Low Reynolds Environment

Microorganisms such as algae and bacteria move in a viscous environment with extremely low Reynolds ($Re$), where the viscous drag dominates the inertial forces. They have adapted to this environment by developing specialized features such as whole-body deformations and flexible structures such as flagella (with various shapes, sizes, and numbers) that break the symmetry during the motion. In this study, we hypothesize that the changes in the flexibility of the flagella during a cycle of movement impact locomotion dynamics of flagellated locomotion. To test our hypothesis, we developed an autonomous, self-propelled robot with four flexible, multi-segmented flagella actuated together by a single DC motor. The stiffness of the flagella during the locomotion is controlled via a cable-driven mechanism attached to the center of the robot. Experimental assessments of the robot's swimming demonstrate that increasing the flexibility of the flagella during recovery stroke and reducing the flexibility during power stroke improves the swimming performance of the robot. Our results give insight into how these microorganisms manipulate their biological features to propel themselves in low viscous media and are of great interest to biomedical and research applications.

==> bibtex.tex <==
\begin{thebibliography}{10}

\bibitem{ullrich_mobility_2013}
F.~Ullrich, C.~Bergeles, J.~Pokki, O.~Ergeneman, S.~Erni, G.~Chatzipirpiridis,
  S.~PanÃ©, C.~Framme, and B.~J. Nelson, ``Mobility {Experiments} {With}
  {Microrobots} for {Minimally} {Invasive} {Intraocular} {Surgery},'' {\em
  Investigative Ophthalmology \& Visual Science}, vol.~54, pp.~2853--2863, Apr.
  2013.

\bibitem{diller_micro-scale_2013}
E.~Diller and M.~Sitti, ``Micro-{Scale} {Mobile} {Robotics},'' {\em Foundations
  and TrendsÂ® in Robotics}, vol.~2, pp.~143--259, Sept. 2013.
\newblock Publisher: Now Publishers, Inc.

\bibitem{sitti_biomedical_2015}
M.~Sitti, H.~Ceylan, W.~Hu, J.~Giltinan, M.~Turan, S.~Yim, and E.~Diller,
  ``Biomedical {Applications} of {Untethered} {Mobile} {Milli}/{Microrobots},''
  {\em Proceedings of the IEEE}, vol.~103, pp.~205--224, Feb. 2015.
\newblock Conference Name: Proceedings of the IEEE.

\bibitem{kozielski_nonresonant_2021}
K.~L. Kozielski, A.~Jahanshahi, H.~B. Gilbert, Y.~Yu, Ã.~Erin, D.~Francisco,
  F.~Alosaimi, Y.~Temel, and M.~Sitti, ``Nonresonant powering of injectable
  nanoelectrodes enables wireless deep brain stimulation in freely moving
  mice,'' {\em Science Advances}, vol.~7, p.~eabc4189, Jan. 2021.
\newblock Publisher: American Association for the Advancement of Science.

\bibitem{nelson_microrobots_2010}
B.~J. Nelson, I.~K. Kaliakatsos, and J.~J. Abbott, ``Microrobots for
  {Minimally} {Invasive} {Medicine},'' {\em Annual Review of Biomedical
  Engineering}, vol.~12, no.~1, pp.~55--85, 2010.
\newblock \_eprint: https://doi.org/10.1146/annurev-bioeng-010510-103409.

\bibitem{ergeneman_magnetically_2008}
O.~Ergeneman, G.~Dogangil, M.~P. Kummer, J.~J. Abbott, M.~K. Nazeeruddin, and
  B.~J. Nelson, ``A {Magnetically} {Controlled} {Wireless} {Optical} {Oxygen}
  {Sensor} for {Intraocular} {Measurements},'' {\em IEEE Sensors Journal},
  vol.~8, pp.~29--37, Jan. 2008.
\newblock Conference Name: IEEE Sensors Journal.

\bibitem{aziz_medical_2020}
A.~Aziz, S.~Pane, V.~Iacovacci, N.~Koukourakis, J.~Czarske, A.~Menciassi,
  M.~Medina-SÃ¡nchez, and O.~G. Schmidt, ``Medical {Imaging} of {Microrobots}:
  {Toward} {In} {Vivo} {Applications},'' {\em ACS Nano}, vol.~14,
  pp.~10865--10893, Sept. 2020.
\newblock Publisher: American Chemical Society.

\bibitem{wang_microrobots_2023}
Y.~Wang, J.~Shen, S.~Handschuh-Wang, M.~Qiu, S.~Du, and B.~Wang, ``Microrobots
  for {Targeted} {Delivery} and {Therapy} in {Digestive} {System},'' {\em ACS
  Nano}, vol.~17, pp.~27--50, Jan. 2023.
\newblock Publisher: American Chemical Society.

\bibitem{gao_synthetic_2014}
W.~Gao and J.~Wang, ``Synthetic micro/nanomotors in drug delivery,'' {\em
  Nanoscale}, vol.~6, pp.~10486--10494, Aug. 2014.
\newblock Publisher: The Royal Society of Chemistry.

\bibitem{dogangil_toward_2008}
G.~Dogangil, O.~Ergeneman, J.~J. Abbott, S.~Pane, H.~Hall, S.~Muntwyler, and
  B.~J. Nelson, ``Toward targeted retinal drug delivery with wireless magnetic
  microrobots,'' in {\em 2008 {IEEE}/{RSJ} {International} {Conference} on
  {Intelligent} {Robots} and {Systems}}, pp.~1921--1926, Sept. 2008.
\newblock ISSN: 2153-0866.

\bibitem{lee_multifunctional_nodate}
Y.-W. Lee, J.-K. Kim, U.~Bozuyuk, N.~O. Dogan, M.~T.~A. Khan, A.~Shiva, A.-M.
  Wild, and M.~Sitti, ``Multifunctional {3D}-{Printed} {Pollen}
  {Grain}-{Inspired} {Hydrogel} {Microrobots} for {On}-{Demand} {Anchoring} and
  {Cargo} {Delivery},'' {\em Advanced Materials}, vol.~n/a, no.~n/a,
  p.~2209812.
\newblock \_eprint:
  https://onlinelibrary.wiley.com/doi/pdf/10.1002/adma.202209812.

\bibitem{yim_biopsy_2014}
S.~Yim, E.~Gultepe, D.~H. Gracias, and M.~Sitti, ``Biopsy using a {Magnetic}
  {Capsule} {Endoscope} {Carrying}, {Releasing}, and {Retrieving} {Untethered}
  {Microgrippers},'' {\em IEEE transactions on bio-medical engineering},
  vol.~61, pp.~513--521, Feb. 2014.

\bibitem{dubowsky_concept_2005}
S.~Dubowsky, K.~Iagnemma, S.~Liberatore, D.~M. Lambeth, J.~S. Plante, and P.~J.
  Boston, ``A Concept Mission: Microbots for Large at Scale
  Planetary Surface and Subsurface Exploration,'' {\em AIP Conference
  Proceedings}, vol.~746, pp.~1449--1458, Feb. 2005.
\newblock Publisher: American Institute of Physics.

\bibitem{yoshimitsu_micro-hopping_2003}
T.~Yoshimitsu, T.~Kubota, I.~Nakatani, T.~Adachi, and H.~Saito, ``Micro-hopping
  robot for asteroid exploration,'' {\em Acta Astronautica}, vol.~52,
  pp.~441--446, Jan. 2003.

\bibitem{chen_biologically_2017}
Y.~Chen, H.~Wang, E.~F. Helbling, N.~T. Jafferis, R.~Zufferey, A.~Ong, K.~Ma,
  N.~Gravish, P.~Chirarattananon, M.~Kovac, and R.~J. Wood, ``A biologically
  inspired, flapping-wing, hybrid aerial-aquatic microrobot,'' {\em Science
  Robotics}, vol.~2, p.~eaao5619, Oct. 2017.
\newblock Publisher: American Association for the Advancement of Science.

\bibitem{yoshida_marangoni-propulsion_2022}
K.~Yoshida and H.~Onoe, ``Marangoni-{Propulsion} {Micro}-{Robots} {Integrated}
  with a {Wireless} {Photonic} {Colloidal} {Crystal} {Hydrogel} {Sensor} for
  {Exploring} the {Aquatic} {Environment},'' {\em Advanced Intelligent
  Systems}, vol.~4, no.~5, p.~2100248, 2022.
\newblock \_eprint:
  https://onlinelibrary.wiley.com/doi/pdf/10.1002/aisy.202100248.

\bibitem{sitti_microscale_2007}
M.~Sitti, ``Microscale and nanoscale robotics systems [{Grand} {Challenges} of
  {Robotics}],'' {\em IEEE Robotics \& Automation Magazine}, vol.~14,
  pp.~53--60, Mar. 2007.
\newblock Conference Name: IEEE Robotics \& Automation Magazine.

\bibitem{dragomir_microrobotics_2014}
F.~Dragomir and O.~E. Dragomir, ``Microrobotics: {Present}, challenges,
  perspectives,'' in {\em 2014 {IEEE} {International} {Conference} on
  {Robotics} and {Biomimetics} ({ROBIO} 2014)}, pp.~1904--1909, Dec. 2014.

\bibitem{qin_micro-forming_2006}
Y.~Qin, ``Micro-forming and miniature manufacturing systems â€” development
  needs and perspectives,'' {\em Journal of Materials Processing Technology},
  vol.~177, pp.~8--18, July 2006.

\bibitem{wang_moisture_2021}
Y.~Wang, M.~Dai, H.~Wu, L.~Xu, T.~Zhang, W.~Chen, Z.~L. Wang, and Y.~Yang,
  ``Moisture induced electricity for self-powered microrobots,'' {\em Nano
  Energy}, vol.~90, p.~106499, Dec. 2021.

\bibitem{huang_adaptive_2019}
H.-W. Huang, F.~E. Uslu, P.~Katsamba, E.~Lauga, M.~S. Sakar, and B.~J. Nelson,
  ``Adaptive locomotion of artificial microswimmers,'' {\em Science Advances},
  vol.~5, p.~eaau1532, Jan. 2019.
\newblock Publisher: American Association for the Advancement of Science.

\bibitem{purcell_efficiency_1997}
E.~M. Purcell, ``The efficiency of propulsion by a rotatingâ€‰flagellum,'' {\em
  Proceedings of the National Academy of Sciences}, vol.~94, pp.~11307--11311,
  Oct. 1997.
\newblock Publisher: Proceedings of the National Academy of Sciences.

\bibitem{zhang_artificial_2010}
L.~Zhang, K.~E.Â Peyer, and B.~J.Â Nelson, ``Artificial bacterial flagella for
  micromanipulation,'' {\em Lab on a Chip}, vol.~10, no.~17, pp.~2203--2215,
  2010.
\newblock Publisher: Royal Society of Chemistry.

\bibitem{begey_manipulability_2020}
J.~Begey, M.~EtiÃ©vant, J.~E. Quispe, A.~Bolopion, M.~Vedrines, J.~Abadie,
  S.~RÃ©gnier, N.~Andreff, and P.~Renaud, ``A {Manipulability} {Criterion} for
  {Magnetic} {Actuation} of {Miniature} {Swimmers} {With} {Flexible}
  {Flagellum},'' {\em IEEE Robotics and Automation Letters}, vol.~5,
  pp.~4891--4898, July 2020.
\newblock Conference Name: IEEE Robotics and Automation Letters.

\bibitem{khalil_controllable_2018}
I.~S.~M. Khalil, A.~F. Tabak, M.~A. Seif, A.~Klingner, and M.~Sitti,
  ``Controllable switching between planar and helical flagellar swimming of a
  soft robotic sperm,'' {\em PLOS ONE}, vol.~13, p.~e0206456, Nov. 2018.
\newblock Publisher: Public Library of Science.

\bibitem{purcell_life_1977}
E.~M. Purcell, ``Life at low {Reynolds} number,'' {\em American Journal of
  Physics}, vol.~45, pp.~3--11, Jan. 1977.
\newblock Publisher: American Association of Physics Teachers.

\bibitem{cohen_swimming_2010}
N.~Cohen and J.~H. Boyle, ``Swimming at low {Reynolds} number: a beginners
  guide to undulatory locomotion,'' {\em Contemporary Physics}, vol.~51,
  pp.~103--123, Mar. 2010.
\newblock Publisher: Taylor \& Francis \_eprint:
  https://doi.org/10.1080/00107510903268381.

\bibitem{ghanbari_bioinspired_2020}
A.~Ghanbari, ``Bioinspired reorientation strategies for application in
  micro/nanorobotic control,'' {\em Journal of Micro-Bio Robotics}, vol.~16,
  pp.~173--197, Dec. 2020.

\bibitem{wan_synchrony_2020}
K.~Y. Wan, ``Synchrony and symmetry-breaking in active flagellar
  coordination,'' {\em Philosophical Transactions of the Royal Society B:
  Biological Sciences}, vol.~375, p.~20190393, Feb. 2020.
\newblock Publisher: Royal Society.

\bibitem{nakamura_flagella-driven_2019}
S.~Nakamura and T.~Minamino, ``Flagella-{Driven} {Motility} of {Bacteria},''
  {\em Biomolecules}, vol.~9, p.~279, July 2019.

\bibitem{wang_flagellar_nodate}
Z.~Wang, A.~Klingner, V.~Magdanz, M.~W. Hoppenreijs, S.~Misra, and I.~S.~M.
  Khalil, ``Flagellar {Propulsion} of {Sperm} {Cells} {Against} a
  {Time}-{Periodic} {Interaction} {Force},'' {\em Advanced Biology}, vol.~n/a,
  no.~n/a, p.~2200210.
\newblock \_eprint:
  https://onlinelibrary.wiley.com/doi/pdf/10.1002/adbi.202200210.

\bibitem{elgeti_physics_2015}
J.~Elgeti, R.~G. Winkler, and G.~Gompper, ``Physics of microswimmersâ€”single
  particle motion and collective behavior: a review,'' {\em Reports on Progress
  in Physics}, vol.~78, p.~056601, Apr. 2015.
\newblock Publisher: IOP Publishing.

\bibitem{rogowski_heterogeneously_2020}
L.~W. Rogowski, M.~Oxner, J.~Tang, and M.~J. Kim, ``Heterogeneously flagellated
  microswimmer behavior in viscous fluids,'' {\em Biomicrofluidics}, vol.~14,
  p.~024112, Mar. 2020.
\newblock Publisher: American Institute of Physics.

\bibitem{alapan_multifunctional_2020}
Y.~Alapan, U.~Bozuyuk, P.~Erkoc, A.~C. Karacakol, and M.~Sitti,
  ``Multifunctional surface microrollers for targeted cargo delivery in
  physiological blood flow,'' {\em Science Robotics}, vol.~5, p.~eaba5726, May
  2020.
\newblock Publisher: American Association for the Advancement of Science.

\bibitem{dreyfus_microscopic_2005}
R.~Dreyfus, J.~Baudry, M.~L. Roper, M.~Fermigier, H.~A. Stone, and J.~Bibette,
  ``Microscopic artificial swimmers,'' {\em Nature}, vol.~437, pp.~862--865,
  Oct. 2005.
\newblock Number: 7060 Publisher: Nature Publishing Group.

\bibitem{singleton_micro-scale_2011}
J.~Singleton, E.~Diller, T.~Andersen, S.~Regnier, and M.~Sitti, ``Micro-scale
  propulsion using multiple flexible artificial flagella,'' in {\em 2011
  {IEEE}/{RSJ} {International} {Conference} on {Intelligent} {Robots} and
  {Systems}}, pp.~1687--1692, Sept. 2011.
\newblock ISSN: 2153-0866.

\bibitem{du_modeling_2022}
Y.~Du, J.~Lam, K.~Sachanandani, and M.~K. Jawed, ``Modeling the {Locomotion} of
  {Articulated} {Soft} {Robots} in {Granular} {Medium},'' {\em IEEE Robotics
  and Automation Letters}, vol.~7, pp.~6495--6502, July 2022.
\newblock Conference Name: IEEE Robotics and Automation Letters.

\bibitem{ye_rotating_2014}
Z.~Ye, S.~RÃ©gnier, and M.~Sitti, ``Rotating {Magnetic} {Miniature} {Swimming}
  {Robots} {With} {Multiple} {Flexible} {Flagella},'' {\em IEEE Transactions on
  Robotics}, vol.~30, pp.~3--13, Feb. 2014.
\newblock Conference Name: IEEE Transactions on Robotics.

\bibitem{du_simple_2021}
Y.~Du, A.~Miller, and M.~K. Jawed, ``Simple {Flagellated} {Soft} {Robot} for
  {Locomotion} near {Air}-{Fluid} {Interface},'' Mar. 2021.
\newblock arXiv:2103.05712 [cs].

\bibitem{diaz_minimal_2021}
K.~Diaz, T.~L. Robinson, Y.~O. Aydin, E.~Aydin, D.~I. Goldman, and K.~Y. Wan,
  ``A minimal robophysical model of quadriflagellate self-propulsion,'' {\em
  Bioinspiration \& Biomimetics}, vol.~16, p.~066001, Sept. 2021.
\newblock Publisher: IOP Publishing.

\bibitem{hof_magnetic_nodate}
L.~Hof, ``Magnetic actuation of swimming soft microrobots with multiple
  flagella,''

\end{thebibliography}

